LiteTrack: Layer Pruning with Asynchronous Feature Extraction for Lightweight and Efficient Visual Tracking

The recent advancements in transformer-based visual trackers have led to significant progress, attributed to their strong modeling capabilities. However, as performance improves, running latency correspondingly increases, presenting a challenge for real-time robotics applications, especially on edge devices with computational constraints. In response to this, we introduce LiteTrack, an efficient transformer-based tracking model optimized for high-speed operations across various devices. It achieves a more favorable trade-off between accuracy and efficiency than the other lightweight trackers. The main innovations of LiteTrack encompass: 1) asynchronous feature extraction and interaction between the template and search region for better feature fushion and cutting redundant computation, and 2) pruning encoder layers from a heavy tracker to refine the balnace between performance and speed. As an example, our fastest variant, LiteTrack-B4, achieves 65.2% AO on the GOT-10k benchmark, surpassing all preceding efficient trackers, while running over 100 fps with ONNX on the Jetson Orin NX edge device. Moreover, our LiteTrack-B9 reaches competitive 72.2% AO on GOT-10k and 82.4% AUC on TrackingNet, and operates at 171 fps on an NVIDIA 2080Ti GPU. The code and demo materials will be available at https://github.com/TsingWei/LiteTrack.

==> tables/ablation_layer.tex <==
% \usepackage{multirow}
% \usepackage{booktabs}

% \usepackage{multirow}
% \usepackage{booktabs}


\begin{table}
    \centering
    \begin{tabular}{c|cc|cccc}
        \toprule
        \# Total                       & \# FE                         & \# AI                          & \multirow{2}{*}{AO} & \multirow{2}{*}{SR$_{0.5}$} & \multirow{2}{*}{SR$_{0.75}$} & \multirow{2}{*}{\textit{fps}} \\
        \multicolumn{1}{l|}{~ ~Layers} & \multicolumn{1}{l}{~ ~Layers} & \multicolumn{1}{l|}{~ ~Layers} &                     &                             &                              &                               \\
        \midrule
        \multirow{3}{*}{8}             & 6                             & 2                              & 70.3                & 80.4                        & 67.2                         & 188                           \\
                                       & 5                             & 3                              & 69.6                & 78.6                        & 66.2                         & 182                           \\
                                       & 0                             & 8                              & 68.3                & 77.9                        & 64.1                         & 173                           \\
        \midrule
        \multirow{2}{*}{6}             & 4                             & 2                              & 68.0                & 77.5                        & 63.4                         &  242                             \\
                                       & 3                             & 3                              & 68.7                & 78.2                        & 64.2                         &  236                             \\
        \midrule
        \multirow{2}{*}{4}             & 3                             & 1                              & -                   & -                           & -                           &                               \\
                                       & 2                             & 2                              & 65.7                & 75.5                        & 58.9                          &  331                             \\
        \bottomrule
    \end{tabular}
    \caption{   }
\end{table}


% \begin{table}
%     \centering
%     \begin{tabular}{c|cc|cc} 
%     \toprule
%     \# Total Layers    & \# FE Layers & \# AI Layers & AO & {\emph{fps}}  \\ 
%     \midrule
%     \multirow{3}{*}{8} & 8            & 0            &    &      \\
%                        & 6            & 2            &    &      \\
%                        & 5            & 3            &    &      \\ 
%                        \midrule
%     \multirow{2}{*}{6} & 4            & 2            &    &      \\
%                        & 3            & 3            &    &      \\ 
%                        \midrule
%     \multirow{2}{*}{2} & 3            & 1            &    &      \\
%                        & 2            & 2            &    &      \\
%     \bottomrule
%     \end{tabular}
%     \end{table}

==> tables/total.tex <==
\begin{table*}[t]\footnotesize
    \centering

    \vspace{-2mm}
    \setlength{\tabcolsep}{2mm}{
        \resizebox{\textwidth}{!}{
            \begin{tabular}{c|l|c|c ccc c ccc c ccc c cc}
                \toprule
                                                              & \multirow{2}*{Method}               & \multirow{2}*{Source} & \multicolumn{3}{c}{TrackingNet~\cite{trackingnet}} &                         & \multicolumn{3}{c}{LaSOT~\cite{LaSOT}} &     & \multicolumn{3}{c}{GOT-10k$^*$~\cite{GOT10K}} &                         & \multicolumn{2}{c}{Speed (\emph{fps})}                                                                                                                \\
                \cline{4-6}
                \cline{8-10}
                \cline{12-14}
                \cline{16-17}
                                                              &                                     &                       & AUC                                                & P$_{Norm}$              & P                                      &     & AUC                                           & P$_{Norm}$              & P                                      &     & AO                      & SR$_{0.5}$              & SR$_{0.75}$             &     & 2080Ti  & OrinNX   \\
                \midrule[0.5pt]
                \multirow{9}*{\rotatebox{90}{Real-time}}      & \my LiteTrack-B9                    & \my Ours              & \my\sotaBest{82.4}                                 & \my\sotaBest{87.3}      & \my\sotaBest{80.4}                     & \my & \my\sotaBest{67.0}                            & \my\sotaBest{77.0}      & \my\sotaBest{72.7}                     & \my & \my\sotaBest{72.2}      & \my\sotaBest{82.3}      & \my\sotaBest{69.3}      & \my & \my 171 & \my 21.4 \\
                                                              & \my LiteTrack-B8                    & \my Ours              & \my\sotaSecond{81.4}                               & \my\sotaSecond{86.4}    & \my\sotaSecond{79.4}                   & \my & \my\sotaSecond{66.4}                          & \my\sotaSecond{76.4}    & \my\sotaSecond{71.4}                   & \my & \my\sotaSecond{70.4}    & \my\sotaSecond{80.1}    & \my\sotaSecond{66.4}    & \my & \my 190 & \my 24.8 \\
                                                              & \my LiteTrack-B6                    & \my Ours              & \my\sotaThird{80.8}                                & \my\sotaThird{85.7}     & \my\sotaThird{78.2}                    & \my & \my\sotaThird{64.6}                           & \my\sotaThird{73.9}     & \my\sotaThird{68.9}                    & \my & \my\sotaThird{68.7}     & \my\sotaThird{78.2}     & \my\sotaThird{64.2}     & \my & \my 237 & \my 31.5 \\
                                                              & \my LiteTrack-B4                    & \my Ours              & \my 79.9                                           & \my 84.9                & \my 76.6                               & \my & \my 62.5                                      & \my 72.1                & \my 65.7                               & \my & \my 65.2                & \my 74.7                & \my 57.7                & \my & \my 315 & \my 44.1 \\
                                                              & HiT-Base\footnotemark[1]~\cite{HiT} & ICCV'23               & 80.0                                               & 84.4                    & 77.3                                   &     & \sotaThird{64.6}                              & 73.3                    & 68.1                                   &     & \nGOT{64.0}             & \nGOT{72.1}             & \nGOT{58.1}             &     & 175     & -        \\
                %   & MixFormerV2-S                       & 75.8                                               & 81.1                                               & 70.4                                               &                     & 60.6                                               & 69.9                                               & 60.4                                               &                     & 62.1                                               & -                                                  & -                                                  &                     & 325                    & 68                    \\
                                                              & E.T.Track~\cite{ETTrack}            & WACV'23               & 75.0                                               & 80.3                    & 70.6                                   &     & 59.1                                          & -                       & -                                      &     & -                       & -                       & -                       &     & 67      & 20.5     \\
                                                              & FEAR-XS~\cite{borsuk2022fear}       & ECCV'22               & -                                                  & -                       & -                                      &     & 53.5                                          & -                       & 54.5                                   &     & \nGOT{61.9}             & \nGOT{72.2}             & -                       &     & 182     & 49.7     \\
                                                              & HCAT~\cite{chen2022efficient}       & ECCVW'22              & 76.6                                               & 82.6                    & 72.9                                   &     & 59.3                                          & 68.7                    & 61.0                                   &     & \nGOT{65.1}             & \nGOT{76.5}             & \nGOT{56.7}             &     & 235     & 33.8     \\
                %   & E.T.Track~\cite{ETTrack}            & WACV'23               & 75.0                                               & 80.3                    & 70.6                                   &     & 59.1                                          & -                       & -                                      &     & -                       & -                       & -                       &     & 67.1      & 20     \\
                                                              & LightTrack~\cite{yan2021lighttrack} & CVPR'21               & 72.5                                               & 77.8                    & 69.5                                   &     & 53.8                                          & -                       & 53.7                                   &     & \nGOT{61.1}             & \nGOT{71.0}             & -                       &     & 107     & 37.6     \\
                                                              & HiFT~\cite{hift,2023SOTsurvey}       & ICCV'21               & 66.7                                               & 73.8                    & 60.9                                   &     & 45.1                                          & 52.7                    & 42.1                                   &     & -                       & -                       & -                       &     & 230     & 50.1     \\
                  & ECO~\cite{danelljan2017eco}         & CVPR'17               & 55.4                                               & 61.8                    & 49.2                                   &     & 32.4                                          & 33.8                    & 30.1                                   &     & 39.5                    & 40.7                    & 17.0                    &     & 113       & 21.9        \\
                \midrule[0.5pt]
                \multirow{10}*{\rotatebox{90}{Non-real-time}} & ARTrack-256~\cite{ARTrack}          & CVPR'23               & \underline{\emph{84.2}}                            & \emph{\underline{88.7}} & 83.5                                   &     & \emph{\underline{70.4}}                       & \emph{\underline{79.5}} & \emph{\underline{76.6}}                &     & \emph{\underline{73.5}} & 82.2                    & \emph{\underline{70.9}} &     & 37      & 5.6      \\
                                                              & GRM-256~\cite{GRM}                  & CVPR'23               & 84.0                                               & \emph{\underline{88.7}} & 83.3                                   &     & 69.9                                          & 79.3                    & 75.8                                   &     & 73.4                    & \emph{\underline{82.9}} & 70.4                    &     & 79      & 10.1     \\
                                                              & OSTrack-256~\cite{ostrack}          & ECCV'22               & 83.1                                               & 87.8                    & 82.0                                   &     & 69.1                                          & 78.7                    & 75.2                                   &     & 71.0                    & 80.4                    & 68.2                    &     & 140     & 18.0     \\
                                                              & MixFormer~\cite{mixformer}          & CVPR'22               & 83.1                                               & 88.1                    & 81.6                                   &     & 69.2                                          & 78.7                    & 74.7                                   &     & 70.7                    & 80.0                    & 67.8                    &     & 48      & 11.8     \\
                                                              & Sim-B/16~\cite{simtrack}            & ECCV'22               & 82.3                                               & 86.5                    & -                                      &     & 69.3                                          & 78.5                    & -                                      &     & 68.6                    & 78.9                    & 62.4                    &     & 131     & 14.6     \\
                                                              & STARK-ST50~\cite{Stark}             & ICCV'21               & 81.3                                               & 86.1                    & -                                      &     & 66.6                                          & -                       & -                                      &     & 68.0                    & 77.7                    & 62.3                    &     & 61      & 13.0     \\
                                                              & TransT~\cite{TransT}                & CVPR'21               & 81.4                                               & 86.7                    & 80.3                                   &     & 64.9                                          & 73.8                    & 69.0                                   &     & 67.1                    & 76.8                    & 60.9                    &     & 84      & 13.3     \\
                                                              & TrDiMP~\cite{wang2021transformer}   & CVPR'21               & 78.4                                               & 83.3                    & 73.1                                   &     & 63.9                                          & -                       & 61.4                                   &     & 67.1                    & 77.7                    & 58.3                    &     & 36      & 6.0      \\
                %   & TrSiam~\cite{wang2021transformer}   & CVPR'21                 & 78.1                                            & 82.9                                            & 72.7                                            &                     & 62.4                                            & -                                               & 60.6                                            &                     & 67.3                                               & 78.7                                               & 58.6                                               &                     & 42                     & 10                    \\
                                                              & PrDiMP~\cite{PrDiMP}                & CVPR'20               & 75.8                                               & 81.6                    & 70.4                                   &     & 59.8                                          & 68.8                    & 60.8                                   &     & 63.4                    & 73.8                    & 54.3                    &     & 47      & 11.6     \\
                                                              & DiMP~\cite{DiMP}                    & ICCV'19               & 74.0                                               & 80.1                    & 68.7                                   &     & 56.9                                          & 65.0                    & 56.7                                   &     & 61.1                    & 71.7                    & 49.2                    &     & 100     & 16.3     \\
                                                              & SiamRPN++~\cite{SiamRPNplusplus}    & CVPR'19               & 73.3                                               & 80.0                    & 69.4                                   &     & 49.6                                          & 56.9                    & 49.1                                   &     & 51.7                    & 61.6                    & 32.5                    &     & 83      & 16.0     \\
                                                              & ATOM~\cite{ATOM}                    & CVPR'19               & 70.3                                               & 77.1                    & 64.8                                   &     & 51.5                                          & 57.6                    & 50.5                                   &     & \nGOT{55.6}             & \nGOT{63.4}             & \nGOT{40.2}             &     & 175     & 15.4     \\
                \bottomrule
            \end{tabular}
        }}
    \caption{State-of-the-art comparison on TrackingNet~\cite{trackingnet}, LaSOT~\cite{LaSOT}, and GOT-10k~\cite{GOT10K} benchmarks.  The best three real-time results are shown in \sotaBest{red}, \sotaSecond{blue} and \sotaThird{green} fonts, and the best non-real-time results are shown in \underline{\emph{underline}} font. * denotes results on GOT-10k obtained following the official one-shot protocol, with \textcolor{gray!60}{gray} font indicating training using extra data.
        % We also report the result on GOT-10k without extra training data in Tab.~\ref{tab:speed}.
    }
    \label{tab:sota}
    \vspace{-4mm}
\end{table*}

==> tables/total_my.tex <==
\begin{table*}[t]\footnotesize
  \centering

  \vspace{-2mm}
  \setlength{\tabcolsep}{2mm}{
      \resizebox{\textwidth}{!}{
          \begin{tabular}{c|l|c ccc c ccc c ccc c cc}
              \toprule
                                                            & \multirow{2}*{Method}               & \multicolumn{3}{c}{TrackingNet}                 &                                                 & \multicolumn{3}{c}{LaSOT}                       &                     & \multicolumn{3}{c}{GOT-10k\dag}                 &                                                 & \multicolumn{2}{c}{Speed (\emph{fps})}                                                                                                                                                                                                                                                                      \\
              \cline{3-5}
              \cline{7-9}
              \cline{11-13}
              \cline{15-16}
                                                            &                                     & AUC                                             & P$_{Norm}$                                      & P                                               &                     & AUC                                             & P$_{Norm}$                                      & P                                               &                     & AO                                                 & SR$_{0.5}$                                         & SR$_{0.75}$                                        &                     & 2080Ti                 & AGX                   \\
              \midrule[0.5pt]
              \multirow{9}*{\rotatebox{90}{Real-time}}      & \cellcolor{gray!15}LiteTrack-B9     & \cellcolor{gray!15}\textbf{\textcolor{cRed}{-}} & \cellcolor{gray!15}\textbf{\textcolor{cRed}{-}} & \cellcolor{gray!15}\textbf{\textcolor{cRed}{-}} & \cellcolor{gray!15} & \cellcolor{gray!15}\textbf{\textcolor{cRed}{-}} & \cellcolor{gray!15}\textbf{\textcolor{cRed}{-}} & \cellcolor{gray!15}\textbf{\textcolor{cRed}{-}} & \cellcolor{gray!15} & \cellcolor{gray!15}\textbf{\textcolor{cRed}{72.2}} & \cellcolor{gray!15}\textbf{\textcolor{cRed}{82.3}} & \cellcolor{gray!15}\textbf{\textcolor{cRed}{69.3}} & \cellcolor{gray!15} & \cellcolor{gray!15}168 & \cellcolor{gray!15}31 \\
                                                            & \cellcolor{gray!15}LiteTrack-B8     & \cellcolor{gray!15}\textcolor{blue}{-}          & \cellcolor{gray!15}\textcolor{cGreen}{-}        & \cellcolor{gray!15}\textcolor{blue}{-}          & \cellcolor{gray!15} & \cellcolor{gray!15}\textcolor{blue}{-}          & \cellcolor{gray!15}\textcolor{cGreen}{-}        & \cellcolor{gray!15}\textcolor{blue}{-}          & \cellcolor{gray!15} & \cellcolor{gray!15}\textcolor{blue}{70.3}          & \cellcolor{gray!15}\textcolor{blue}{80.4}          & \cellcolor{gray!15}\textcolor{blue}{67.2}          & \cellcolor{gray!15} & \cellcolor{gray!15}188 & \cellcolor{gray!15}35 \\
                                                            & \cellcolor{gray!15}LiteTrack-B6     & \cellcolor{gray!15}-                            & \cellcolor{gray!15}-                            & \cellcolor{gray!15}-                            & \cellcolor{gray!15} & \cellcolor{gray!15}64.6                         & \cellcolor{gray!15}73.9                         & \cellcolor{gray!15}68.9                         & \cellcolor{gray!15} & \cellcolor{gray!15}\textcolor{cGreen}{69.7}        & \cellcolor{gray!15}\textcolor{cGreen}{78.9}        & \cellcolor{gray!15}\textcolor{cGreen}{64.5}        & \cellcolor{gray!15} & \cellcolor{gray!15}236 & \cellcolor{gray!15}41 \\
                                                            & \cellcolor{gray!15}LiteTrack-B4     & \cellcolor{gray!15}79.9                         & \cellcolor{gray!15}84.9                         & \cellcolor{gray!15}76.6                         & \cellcolor{gray!15} & \cellcolor{gray!15}-                            & \cellcolor{gray!15}-                            & \cellcolor{gray!15}-                            & \cellcolor{gray!15} & \cellcolor{gray!15}66.7                            & \cellcolor{gray!15}76.1                            & \cellcolor{gray!15}60.8                            & \cellcolor{gray!15} & \cellcolor{gray!15}331 & \cellcolor{gray!15}56 \\
              %\cline{2-17}
                                                            & HiT-Base~\cite{HiT}                 & 80.0                                            & 84.4                                            & 77.3                                            &                     & 64.6                                            & 73.3                                            & 68.1                                            &                     & 64.0                                               & 72.1                                               & 58.1                                               &                     & 175$^*$                & 61                    \\
              %   & MixFormerV2-S                       & 75.8                                               & 81.1                                               & 70.4                                               &                     & 60.6                                               & 69.9                                               & 60.4                                               &                     & 62.1                                               & -                                                  & -                                                  &                     & 325                    & 68                    \\
                                                            & FEAR-XS~\cite{borsuk2022fear}       & -                                               & -                                               & -                                               &                     & 53.5                                            & -                                               & 54.5                                            &                     & 61.9                                               & 72.2                                               & -                                                  &                     & 113                    & 38                    \\
                                                            & HCAT~\cite{chen2022efficient}       & 76.6                                            & 82.6                                            & 72.9                                            &                     & 59.3                                            & 68.7                                            & 61.0                                            &                     & 65.1                                               & 76.5                                               & 56.7                                               &                     & 201                    & 55                    \\
                                                            & E.T.Track~\cite{ETTrack}            & 75.0                                            & 80.3                                            & 70.6                                            &                     & 59.1                                            & -                                               & -                                               &                     & -                                                  & -                                                  & -                                                  &                     & 57                     & 20                    \\
                                                            & LightTrack~\cite{yan2021lighttrack} & 72.5                                            & 77.8                                            & 69.5                                            &                     & 53.8                                            & -                                               & 53.7                                            &                     & 61.1                                               & 71.0                                               & -                                                  &                     & 138                    & 36                    \\
                                                            & ATOM~\cite{ATOM}                    & 70.3                                            & 77.1                                            & 64.8                                            &                     & 51.5                                            & 57.6                                            & 50.5                                            &                     & 55.6                                               & 63.4                                               & 40.2                                               &                     & 87                     & 22                    \\
                                                            & ECO~\cite{danelljan2017eco}         & 55.4                                            & 61.8                                            & 49.2                                            &                     & 32.4                                            & 33.8                                            & 30.1                                            &                     & 31.6                                               & 30.9                                               & 11.1                                               &                     & 255                    & 39                    \\
              \midrule[0.5pt]
              %
              \multirow{10}*{\rotatebox{90}{Non-real-time}} & ARTrack-256~\cite{ARTrack}          & \underline{\emph{84.2}}                         & \emph{\underline{88.7}}                         & 83.5                                            &                     & \emph{\underline{70.4}}                         & \emph{\underline{79.5}}                         & \emph{\underline{76.6}}                         &                     & \emph{\underline{73.5}}                            & 82.2                                               & \emph{\underline{70.9}}                            &                     & 63                     & 9                     \\
                                                            & GRM-256~\cite{GRM}                  & 84.0                                            & \emph{\underline{88.7}}                         & 83.3                                            &                     & 69.9                                            & 79.3                                            & 75.8                                            &                     & 73.4                                               & \emph{\underline{82.9}}                            & 70.4                                               &                     & 82                     & 12                    \\
                                                            & OSTrack-256~\cite{ostrack}          & 83.1                                            & 87.8                                            & 82.0                                            &                     & 69.1                                            & 78.7                                            & 75.2                                            &                     & 71.0                                               & 80.4                                               & 68.2                                               &                     & 117                    & 19                    \\
              %
                                                            & MixFormer~\cite{mixformer}          & 83.1                                            & 88.1                                            & 81.6                                            &                     & 69.2                                            & 78.7                                            & 74.7                                            &                     & 70.7                                               & 80.0                                               & 67.8                                               &                     & 75                     & 12                    \\
                                                            & Sim-B/16~\cite{simtrack}            & 82.3                                            & -                                               & \emph{\underline{86.5}}                         &                     & 69.3                                            & 78.5                                            & -                                               &                     & 68.6                                               & 78.9                                               & 62.4                                               &                     & 87                     & 16                    \\
                                                            & STARK-ST50~\cite{Stark}             & 81.3                                            & 86.1                                            & -                                               &                     & 66.6                                            & -                                               & -                                               &                     & 68.0                                               & 77.7                                               & 62.3                                               &                     & 54                     & 13                    \\
                                                            & TransT~\cite{TransT}                & 81.4                                            & 86.7                                            & 80.3                                            &                     & 64.9                                            & 73.8                                            & 69.0                                            &                     & 72.3                                               & 82.4                                               & 68.2                                               &                     & 67                     & 13                    \\
                                                            & TrDiMP~\cite{wang2021transformer}   & 78.4                                            & 83.3                                            & 73.1                                            &                     & 63.9                                            & -                                               & 61.4                                            &                     & 68.8                                               & 80.5                                               & 59.7                                               &                     & 44                     & 10                    \\
                                                            & TrSiam~\cite{wang2021transformer}   & 78.1                                            & 82.9                                            & 72.7                                            &                     & 62.4                                            & -                                               & 60.6                                            &                     & 67.3                                               & 78.7                                               & 58.6                                               &                     & 42                     & 10                    \\
                                                            & PrDiMP~\cite{PrDiMP}                & 75.8                                            & 81.6                                            & 70.4                                            &                     & 59.8                                            & 68.8                                            & 60.8                                            &                     & 63.4                                               & 73.8                                               & 54.3                                               &                     & 47                     & 11                    \\
                                                            & DiMP~\cite{DiMP}                    & 74.0                                            & 80.1                                            & 68.7                                            &                     & 56.9                                            & 65.0                                            & 56.7                                            &                     & 61.1                                               & 71.7                                               & 49.2                                               &                     & 77                     & 17                    \\
                                                            & SiamRPN++~\cite{SiamRPNplusplus}    & 73.3                                            & 80.0                                            & 69.4                                            &                     & 49.6                                            & 56.9                                            & 49.1                                            &                     & 51.7                                               & 61.6                                               & 32.5                                               &                     & 56                     & 11                    \\
              \bottomrule
          \end{tabular}
      }}
  \caption{State-of-the-art comparison on TrackingNet~\cite{trackingnet}, LaSOT~\cite{LaSOT}, and GOT-10k~\cite{GOT10K} benchmarks. We use \textcolor{gray}{gray} color to denote our trackers. The best three real-time results are shown in \textbf{\textcolor{cRed}{red}}, \textcolor{blue}{blue} and \textcolor{cGreen}{green} fonts, and the best non-real-time results are shown in \underline{\emph{underline}} font. * indicates that the speed is obtained from the paper with a stronger GPU since the code is not yet public available. \dag indicates that only non-real-time trackers report the performance on GOT-10k following the official one-shot protocol, while the real-time trackers not.  We also report the result on GOT-10k without extra training data in Tab.~\ref{tab:speed}.}
  \label{tab:sota}
  \vspace{-2.5mm}
\end{table*}
